Linear time algorithms for Clobber

We prove that the single-player game clobber is solvable in linear time when played on a line or on a cycle. For this purpose, we show that this game is equivalent to an optimization problem on a set of words defined by seven classes of forbidden patterns. We also prove that, playing on the cycle, it is always possible to remove at least 2n/3 pawns, and we give a conformation for which it is not possible to do better, answering questions recently asked by Faria et al.

==> conclusions.tex <==
\section{Conclusions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper, we have shown that playing solitaire Clobber on a
line or a circle can be viewed as an optimization problem on a set
of words with forbidden patterns. This equivalence has allowed us
to design a linear-time algorithm computing the reducibility value
of an initial conformation and providing an optimal strategy, for
both the cycle and the line. This linear complexity is clearly
optimal as reading the initial conformation already requires $n$
operations. Using this forbidden pattern approach and a simple
alternative algorithm, we were also able to easily prove that the
maximal possible reducibility value on a cycle is $n/3 + O(1)$.

It remains open to determine to which extend our approach can be applied to other topologies. On a general graph, one
can build a \quotes{word} corresponding to a game of solitaire \RMJ{C}lobber by assigning a symbol to every edge, in the same way as we do for each separation between
positions. This is however most probably ineffective in the
general case, as computing the reducibility value is known to be
NP-\RMJ{complete} for general graphs \cite{clobber_duchene}.


==> declarations.tex <==
\bibliographystyle{plain}


\usepackage{clobber}
\usepackage{amssymb,amsmath}
\usepackage{amsfonts}
\usepackage[english]{babel}
%\usepackage[french]{babel}
\usepackage[latin1]{inputenc}
\usepackage{fancyhdr}
\usepackage{yfonts}
\usepackage{mathrsfs}
\usepackage[dvips]{graphicx}
\usepackage[rflt]{floatflt}
%\usepackage{amsthm}
\usepackage{cite}
\usepackage{latexsym}

\usepackage{algorithm}
\floatname{algorithm}{Alg.}
\usepackage{algorithmic}
\usepackage{psfrag}

\newtheorem{defi}{Definition}




\newcommand{\JMH}[1]{#1}
\newcommand{\JMHB}[1]{#1}
\newcommand{\RMJ}[1]{#1}



\providecommand{\prt}[1]{\left( #1 \right)}
\providecommand{\C}{\mathbb{C}} \providecommand{\PP}{\mathbb{P}}
\providecommand{\e}{\phantom{aaa}}
\providecommand{\pe}{\phantom{a}} \providecommand{\F}{\mathscr{F}}
\providecommand{\Lap}[1]{\mathscr{L}\prt{#1}}
\providecommand{\Lapinv}[1]{\mathscr{L}^{-1}\prt{#1}}

\providecommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}

\providecommand{\derivee}[2]{\frac{\partial #1}{\partial #2}}
\providecommand{\abs[1]}{\left|#1\right|}
\providecommand{\norm[1]}{\abs{\abs{#1}}}

\providecommand{\floor[1]}{\lfloor  #1 \rfloor }
\providecommand{\ceil[1]}{\lceil #1  \rceil}

\providecommand{\comjh[1]}{\com{JH}{#1}}
\providecommand{\comrj[1]}{\com{RJ}{#1}}

\providecommand{\com[2]}{\begin{tt}[#1: #2]\end{tt}}
\providecommand{\quotes[1]}{``#1"}
\providecommand{\T}{\mathcal{T}}%
\renewcommand{\S}{\mathcal{S}}%
\providecommand{\A}{\mathcal{A}}%
\providecommand{\X}{\mathcal{X}}%
\providecommand{\Y}{\mathcal{Y}}%

\providecommand{\temprem[1]}{#1}

\providecommand{\clob[1]}{\clobber{#1}\phantom{#1}}



\providecommand{\clobstat}[2]{\frac{#1}{#2}}


%\providecommand{\nomove}[1]{\overline{#1}}
\providecommand{\nomove}[1]{\overline{#1}}
%\providecommand{\indetsep}{.\phantom{a}.}
%\providecommand{\indetsep}{X}
\providecommand{\indetsep}{x} \providecommand{\samepawns}{s}
\providecommand{\difpawns}{a}

%\providecommand{\Rx}{\overrightarrow{\indetsep}}%
%\providecommand{\RI}{\overrightarrow{I}}%
%\providecommand{\RC}{\overrightarrow{C}}%
%\providecommand{\Lx}{\overleftarrow{\indetsep}}%
%\providecommand{\LI}{\overleftarrow{I}}%
%\providecommand{\LC}{\overleftarrow{C}}%
%\providecommand{\vx}{\nomove{\indetsep}}%
%\providecommand{\vI}{\nomove{I}}%
%\providecommand{\vC}{\nomove{C}}%
%\providecommand{\yx}{\indetsep}%
%\providecommand{\yI}{I}%
%\providecommand{\yC}{C}%

\providecommand{\Rx}{\overrightarrow{\indetsep}}%
\providecommand{\RI}{\overrightarrow{\difpawns}}%
\providecommand{\RC}{\overrightarrow{\samepawns}}%
\providecommand{\Lx}{\overleftarrow{\indetsep}}%
\providecommand{\LI}{\overleftarrow{\difpawns}}%
\providecommand{\LC}{\overleftarrow{\samepawns}}%
\providecommand{\vx}{\nomove{\indetsep}}%
\providecommand{\vI}{\nomove{\difpawns}}%
\providecommand{\vC}{\nomove{\samepawns}}%
\providecommand{\yx}{\indetsep}%
\providecommand{\yI}{\difpawns}%
\providecommand{\yC}{\samepawns}%


%\providecommand{\Rx}{\overrightarrow x}
%\providecommand{\RI}{\overrightarrow I}
%\providecommand{\RC}{\overrightarrow C}
%\providecommand{\Lx}{\overleftarrow x}
%\providecommand{\LI}{\overleftarrow I}
%\providecommand{\LC}{\overleftarrow C}
%\providecommand{\vI}{\breve I}%
%\providecommand{\vC}{\breve C}%
%\providecommand{\vx}{\breve x}%
%\providecommand{\yx}{x}%
%\providecommand{\yI}{I}%
%\providecommand{\yC}{v}


==> intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The combinatorial game Clobber was introduced by Albert, Grossman,
Nowa\-kow\-ski and Wolfe in 2002~\cite{clobb}. It is played with
black and white pawns \RMJ{that are placed on a grid, or more
generally on \RMJ{the nodes of} an undirected graph}. White begins and moves a white
pawn onto an adjacent black pawn and removes this black pawn from
the game. The place formerly occupied by the white pawn is then
empty and cannot be occupied anymore. Then Black plays similarly
with the black pawns, etc. The player making the last move wins
the game. Starting from the following initial
conformation (where pawns lie on a line),
% is for instance winning
%for White
$$\clobber{xoxoxoxo\\},$$
the first play of White could be $\clob{xoxoxoo}$. Black
could follow with $\clob{xoxxaoo}$, after which White could
win by playing $\clob{oaxxaoo}$ as Black would then be unable to
play (It can be proved that with this initial alternate conformation of length $8$, the
first player can always win).  This game has received increasing attention for the last years, and it is for instance possible to play Clobber on the web \cite{clob_site}.


We study here solitaire Clobber, which is a single-player version of this game, introduced by Demaine et al. \cite{clobber_demaine}.

There are two ways to define this one player version. In one
version, the player is forced to play alternatively with white and
black pawns as in the 2-player game.

In a second version, the player can
move a black or a white pawn at each turn.

In both versions of the game, the goal is to remove as many pawns
as possible. The smallest number of remaining pawns that can be
obtained \RMJ{from} a particular initial conformation is called
the \emph{reducibility value} of this conformation. Little is
known about these games except that both are difficult. More
precisely, in both cases it is NP-complete to determine the
reducibility value of a given initial conformation even if the
underlying graph is a simple grid \cite{clobber_demaine,
clobber_duchene}.  We focus on the second version of the solitaire
game, where the player can chose at each turn the color he plays.
In the sequel we simply refer to the second version as
\quotes{solitaire Clobber}.


In \cite{clobber_duchene} Faria et al. prove that the
reducibility value of an initial conformation on a line ($1\times
n$ grid) can be computed in quadratic time and \RMJ{they} ask if an
algorithm with a smaller complexity exists. From \RMJ{their} method, \RMJ{they}
deduce a cubic time algorithm to compute the reducibility value
of conformations on a cycle, which \RMJ{they} conjecture to be \RMJ{never} larger than $n/4+O(1)$. We show in this paper that
the reducibility value of a conformation on both the line and the
cycle can be computed in linear time
%\comjh{check if not $n\log(n)$}
by an algorithm which also provides a sequence of moves attaining
this value. We also exhibit a class of conformations on a cycle
whose reducibility value is $n/3+O(1)$, thus disproving the
conjecture of Faria et al.  We then prove that this is the largest
possible reducibility value for cyclic conformations.


The paper is organized as follows: In Section \ref{section-static}
we reformulate Solitaire Clobber on a line as an optimization
problem over words. \JMHB{We give then} in Section
\ref{section-explo} an algorithm that solves this problem in
$O(n)$ operations \JMHB{and explicitly provides} an optimal
strategy for the given conformation. \JMHB{Finally in Section
\ref{section-cycle} we adapt this algorithm to the cyclic case and
prove that the worst reducibility value on a cycle is $n/3+O(1)$.}

